Multiplex Graph Networks for Multimodal Brain Network Analysis

In this paper, we propose MGNet, a simple and effective multiplex graph convolutional network (GCN) model for multimodal brain network analysis. The proposed method integrates tensor representation into the multiplex GCN model to extract the latent structures of a set of multimodal brain networks, which allows an intuitive 'grasping' of the common space for multimodal data. Multimodal representations are then generated with multiplex GCNs to capture specific graph structures. We conduct classification task on two challenging real-world datasets (HIV and Bipolar disorder), and the proposed MGNet demonstrates state-of-the-art performance compared to competitive benchmark methods. Apart from objective evaluations, this study may bear special significance upon network theory to the understanding of human connectome in different modalities. The code is available at https://github.com/ZhaomingKong/MGNets.

==> Fig_brain_structure.tex <==
\begin{figure}[htbp]
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=2.99in]{Figs/multimodal_graph.png}
  \caption{An example of multimodal brain networks.}
  \vspace{-6pt}
  \label{Fig_brain_structure}
\end{figure}


==> Fig_parameter_K.tex <==
% \begin{figure}[htbp]
% \graphicspath{{Figs/}}
% \centering
% \subfigure[Influence of K and batch size]{
% \label{Fig4}
% \includegraphics[width=1.5in]{BP_parameter_K_batchsize}}
% \subfigure[Influence of K and feature size]{
% \label{Fig4}
% \includegraphics[width=1.68in]{BP_parameter_K_featuresize}}
% \caption{Parameter sensitivity analysis on BP dataset with different batch size, feature size $F$ and $K$ nearest neighbours..}
% \label{Fig_parameter_sensitivity}
% \end{figure}

\begin{figure}[htbp]
\graphicspath{{Figs/}}
\centering
 \vspace{-6pt}
%\subfigure[Number of Neighbors]{
%\includegraphics[width=1.55in, height=1.35in]{Figs/neibour.png}}
%\subfigure[Number of Features]{
%\includegraphics[width=1.55in, height=1.35in]{Figs/features.png}}
\subfigure[HIV (tSNE)]{
\includegraphics[width=1.48in, height=1.36in]{Figs/Fig_visual_embeddings/HIV_embedding_original_DPI_600}}
\subfigure[$\#$ Neighbours]{
\includegraphics[width=1.54in, height=1.354in]{Figs/Fig_parameter_tuning/MGNet_GCN_k_neighbours_HIV.png}}
\caption{(a): tSNE Visualization results of HIV dataset. (b) The influence of $K$ neighbours for MGNet and GCN on the HIV dataset.}
\label{Fig_parameter_K}
\vspace{-8pt}
\end{figure}


==> Fig_parameter_sensitivity.tex <==
% \begin{figure}[htbp]
% \graphicspath{{Figs/}}
% \centering
% \subfigure[Influence of K and batch size]{
% \label{Fig4}
% \includegraphics[width=1.5in]{BP_parameter_K_batchsize}}
% \subfigure[Influence of K and feature size]{
% \label{Fig4}
% \includegraphics[width=1.68in]{BP_parameter_K_featuresize}}
% \caption{Parameter sensitivity analysis on BP dataset with different batch size, feature size $F$ and $K$ nearest neighbours..}
% \label{Fig_parameter_sensitivity}
% \end{figure}

\begin{figure}[htbp]
\graphicspath{{Figs/}}
\centering
%\subfigure[Number of Neighbors]{
%\includegraphics[width=1.55in, height=1.35in]{Figs/neibour.png}}
%\subfigure[Number of Features]{
%\includegraphics[width=1.55in, height=1.35in]{Figs/features.png}}
\subfigure[Feature size]{
\includegraphics[width=1.518in, height=1.318in]{Figs/Fig_parameter_tuning/MGNet_feature_size_three_datasets.png}}
\subfigure[Batch size]{
\includegraphics[width=1.518in, height=1.31
in]{Figs/Fig_parameter_tuning/MGNet_batch_size_three_datasets.png}}
\caption{Parameter sensitivity analysis of {\ours} on HIV, BP and PPMI datasets with varying numbers of features and batch size.}
\label{Fig_parameter_sensitivity}
\vspace{-6pt}
\end{figure}


==> Fig_visual_embeddings.tex <==
% \begin{figure}[htbp]
% \graphicspath{{Figs/Fig_visual_embeddings/}}
% \centering
% \subfigure[MVGCN]{
% \label{Fig4}
% \includegraphics[width=1.38in]{HIV_tSNE_MVGCN}}
% \subfigure[MGNet]{
% \label{Fig4}
% \includegraphics[width=1.38in]{HIV_tSNE_MGNet}}

% \caption{Comparison of the graph embeddings learned by MVGCN and our MGNet on the HIV dataset.}
% \label{Fig_visual_embeddings}
% \end{figure}

% \begin{figure}[htbp]
% \centering
% %\subfigure[Input]{
% %\includegraphics[width=1.02in]{Figs/Fig_visual_embeddings/HIV_tSNE}}
% \subfigure[MVGCN]{
% \includegraphics[width=1.5in, height = 1.352in]{Figs/Fig_visual_embeddings/HIV_embedding_MVGCN_DPI_600}}
% \subfigure[MGNet]{
% \includegraphics[width=1.5in, height = 1.34in]{Figs/Fig_visual_embeddings/HIV_embedding_MGNet_DPI_600}}
% %\subfigure[Batch Size]{
% %\includegraphics[width=1.6in, height=1.1in]{Figs/batch_size.png}}
% % \subfigure[]{
% % \includegraphics[width=1.58in]{Figs/BP_parameter_K.png}}
% % \subfigure[Influence of K and feature size]{
% % \includegraphics[width=1.58in]{Figs/BP_parameter_feature_size.png}}
% \caption{A tSNE visualization of the graph embeddings learned by MVGCN and MGNet on the HIV dataset.}
% \label{Fig_visual_embeddings}
% \vspace{-3pt}
% \end{figure}

\begin{figure}[htbp]
\centering
%\subfigure[Input]{
%\includegraphics[width=1.02in]{Figs/Fig_visual_embeddings/HIV_tSNE}}
\subfigure[MVGCN]{
\includegraphics[width=1.589in, height = 1.508in]{Figs/Fig_visual_embeddings/HIV_tSNE_MVGCN_new2.png}}
\subfigure[MGNet]{
\includegraphics[width=1.59in, height = 1.51in]{Figs/Fig_visual_embeddings/HIV_tSNE_MGNet_new2.png}}
%\subfigure[Batch Size]{
%\includegraphics[width=1.6in, height=1.1in]{Figs/batch_size.png}}
% \subfigure[]{
% \includegraphics[width=1.58in]{Figs/BP_parameter_K.png}}
% \subfigure[Influence of K and feature size]{
% \includegraphics[width=1.58in]{Figs/BP_parameter_feature_size.png}}
\caption{A tSNE visualization of the graph embeddings learned by MVGCN and MGNet on the HIV dataset.}
\label{Fig_visual_embeddings}
\vspace{-3pt}
\end{figure}

==> Fig_visual_original_subjects.tex <==
\begin{figure}[t]
\centering
\subfigure[Subject 1]{
\includegraphics[width=1.52in]{Figs/Fig_Visualize_views/HIV_subj_1_combined}}
\subfigure[Subject 2]{
\includegraphics[width=1.52in]{Figs/Fig_Visualize_views/HIV_subj_2_combined}}
\caption{Original HIV brain network data with two modalities.}
\label{Fig_visual_original_subjects}
\vspace{-10pt}
\end{figure}

==> Fig_visual_weights.tex <==


\begin{wrapfigure}{l}{0.26\textwidth}
  \vspace{-6pt}
  \begin{center}
    \includegraphics[width=0.23\textwidth]{Figs/Fig_visual_weights/Weight_Comparison_new2.png}
  \end{center}
  \caption{\label{Fig_visual_weights} Comparison of learned modality weight $\boldsymbol{\alpha}$ of DTI and fMRI on HIV and BP data.}
  \vspace{-10pt}
\end{wrapfigure}

% \begin{figure}[htbp]
% \centering
% \includegraphics[width=1.58in, height = 1.38in]{Figs/Fig_visual_weights/Weight_Comparison_new2.png}
% \caption{Comparison of learned modality weight $\mathbf{a}$ of DTI and fMRI for HIV and BP data.}
% \label{Fig_visual_weights}
% \vspace{-8pt}
% \end{figure}


==> Fig_visualize_BP_HIV_views.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/Fig_Visualize_views/}}
\centering
\vspace{-5pt}
\subfigure[HIV-DTI]{
\label{Fig4}
\includegraphics[width=0.74in]{HIV_DTI}}
\subfigure[HIV-fMRI]{
\label{Fig4}
\includegraphics[width=0.74in]{HIV_fMRI}}
\subfigure[BP-DTI]{
\label{Fig4}
\includegraphics[width=0.74in]{BP_DTI}}
\subfigure[BP-fMRI]{
\label{Fig4}
\includegraphics[width=0.74in]{BP_fMRI}}
\caption{Visual comparison of two different modalities (DTI and fMRI) on HIV and BP data.}
\label{Fig_visualize_BP_HIV_views}
\vspace{-15pt}
\end{figure}


==> Table_ablation_node_embedding_matrix.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
%\begin{table}[htbp]
%\tiny
%  \centering
%  \caption{Ablation study on the importance of learning node embedding matrix with tensor decomposition.}
%    \begin{tabular}{cccccc}
%    \toprule
%    Dataset & Method & Accracy & AUC   & Sensitivity & Specificity \\
%    \midrule
%    \multirow{3}[5]{*}{HIV} & RandomNode-GCN & 0.629 $\pm$ 0.168  & 0.623 $\pm$ 0.130 & 0.518 $\pm$ 0.347 & 0.730 $\pm$ 0.322 \\
%\cmidrule{2-6}          & Node2Vec-GCN  & 0.671 $\pm$ 0.161 & 0.658 $\pm$ 0.152 & 0.542 $\pm$ 0.343 & \textbf{0.775 $\pm$ 0.286} \\
%\cmidrule{2-6}          & ITD-GCN & \textbf{0.686 $\pm$ 0.128} & \textbf{0.679 $\pm$ 0.099} & \textbf{0.583 $\pm$ 0.297} & \textbf{0.775 $\pm$ 0.286} \\
%    \midrule
%    \multirow{3}[5]{*}{BP} & RandomNode-GCN & 0.778 $\pm$ 0.203 & 0.766 $\pm$ 0.216 & 0.831 $\pm$ 0.140 & 0.702 $\pm$ 0.324 \\
%\cmidrule{2-6}          & Node2Vec-GCN  & 0.833
% $\pm$ 0.105 & \textbf{0.841 $\pm$ 0.114} & 0.831 $\pm$ 0.115 & \textbf{0.852 $\pm$ 0.163} \\
%\cmidrule{2-6}          & ITD-GCN & \textbf{0.833 $\pm$ 0.105} & 0.829 $\pm$ 0.121 & \textbf{0.856 $\pm$ 0.146} & 0.802 $\pm$ 0.191 \\
%    \bottomrule
%    \end{tabular}%
%  \label{Table_ablation_node_embedding_matrix}%
%\end{table}%

% Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[htbp]
% % \tiny
%   \centering
%   \caption{Ablation study on the influence of obtaining node embedding matrix with different methods.}
%     \begin{tabular}{cccc}
%     \toprule
%     Dataset & Method & Accuracy & AUC \\
%     \midrule
%     \midrule
%     \multirow{4}[8]{*}{HIV} & RandomNode-GCN & 0.629 $\pm$ 0.168 & 0.623 $\pm$ 0.130 \\
% \cmidrule{2-4}          & Node2Vec-GCN & 0.671 $\pm$ 0.166 & 0.658 $\pm$ 0.152 \\
% \cmidrule{2-4}          & IT-GCN(CP) & \textbf{0.686 $\pm$ 0.162} & 0.675 $\pm$ 0.142 \\
% \cmidrule{2-4}          & IT-GCN & \textbf{0.686 $\pm$ 0.131} & \textbf{0.679 $\pm$ 0.099} \\
%     \midrule
%     \multirow{4}[8]{*}{BP} & RandomNode-GCN & 0.778 $\pm$ 0.203 & 0.766 $\pm$ 0.216 \\
% \cmidrule{2-4}          & Node2Vec-GCN & 0.833 $\pm$ 0.108 & 0.821 $\pm$ 0.114 \\
% \cmidrule{2-4}          & IT-GCN(CP) & 0.833  $\pm$ 0.094 & 0.829 $\pm$ 0.104 \\
% \cmidrule{2-4}          & IT-GCN & \textbf{0.833 $\pm$ 0.105} & \textbf{0.829 $\pm$ 0.121} \\
%     \bottomrule
%     \end{tabular}%
%   \label{Table_ablation_node_embedding_matrix}%
% \end{table}%

% \begin{table}[htbp]
%   \centering
%   \caption{Ablation study on the influence of obtaining node embedding matrix with different methods.}
%   \resizebox{3.350in}{!}{%
%     \begin{tabular}{ccccc}
%     \toprule
%     Dataset & Method & Accuracy & AUC   & Time (s) \\
%     \midrule
%     \multirow{4}[8]{*}{HIV} & RandomNode-GCN & 0.629 $\pm$ 0.168 & 0.623 $\pm$ 0.130 & 0.06 \\
% \cmidrule{2-5}          & Node2Vec-GCN & 0.671 $\pm$ 0.166 & 0.658 $\pm$ 0.152 & $>$ 3600 \\
% \cmidrule{2-5}          & IT-GCN (CP) & \textbf{0.686 $\pm$ 0.162} & 0.675 $\pm$ 0.142 & 21.8 \\
% \cmidrule{2-5}          & IT-GCN & \textbf{0.686 $\pm$ 0.131} & \textbf{0.679 $\pm$ 0.099} & \textbf{0.18} \\
%     \midrule
%     \multirow{4}[8]{*}{BP} & RandomNode-GCN & 0.778 $\pm$ 0.203 & 0.766 $\pm$ 0.216 & 0.05 \\
% \cmidrule{2-5}          & Node2Vec-GCN & 0.833 $\pm$ 0.108 & 0.821 $\pm$ 0.114 & $>$ 3600 \\
% \cmidrule{2-5}          & IT-GCN (CP) & 0.833  $\pm$ 0.094 & 0.829 $\pm$ 0.104 & 15.4 \\
% \cmidrule{2-5}          & IT-GCN & \textbf{0.833 $\pm$ 0.105} & \textbf{0.829 $\pm$ 0.121} & \textbf{0.26} \\
%     \bottomrule
%     \end{tabular}%
%     }
%   \label{Table_ablation_node_embedding_matrix}%
% \end{table}%



==> Table_results_comparison.tex <==
% Table generated by Excel2LaTeX from sheet 'Use_original_label_division'
%\begin{table*}[htbp]
%  \centering
%  \caption{Comparison of different modeling approaches.}
%    \begin{tabular}{c|c|c|c|c|c}
%    \specialrule{.1em}{.05em}{.05em}
%    Dataset & Method & Accuracy & AUC   & Sensitivity & Specificity \\
%    \hline
%    \multirow{6}[8]{*}{HIV} & PCA & \textbf{0.686 $\pm$ 0.144} & 0.672 $\pm$ 0.175 & \textbf{0.725 $\pm$ 0.306} & 0.620 $\pm$ 0.219 \\
%          & MPCA & 0.643 $\pm$ 0.135 & 0.622 $\pm$ 0.146 & \textbf{0.725 $\pm$ 0.314} & 0.520 $\pm$ 0.189 \\
%          & CNN   & 0.543 $\pm$ 0.158 & 0.540 $\pm$ 0.088 & 0.600 $\pm$ 0.459 & 0.480 $\pm$ 0.509 \\
%          & M2E & 0.586 $\pm$ 0.249 & 0.553 $\pm$ 0.326 & 0.292 $\pm$ 0.292 & \textbf{0.813 $\pm$ 0.179} \\
%          & MIC & 0.443 $\pm$ 0.191 & 0.330 $\pm$ 0.268 & 0.392 $\pm$ 0.348 & 0.445 $\pm$ 0.248 \\
%          & ITD-GCN & \textbf{0.686 $\pm$ 0.128} & \textbf{0.679 $\pm$ 0.099} & 0.583 $\pm$ 0.297 & 0.775 $\pm$ 0.286 \\
%    \hline \hline
%    % \specialrule{.1em}{.05em}{.05em}
%    \multirow{6}[8]{*}{BP} & PCA & 0.544 $\pm$ 0.161 & 0.543 $\pm$ 0.140 & 0.534 $\pm$ 0.259 & 0.552 $\pm$ 0.120 \\
%         & MPCA & 0.522 $\pm$ 0.149 & 0.528 $\pm$ 0.148 & 0.627 $\pm$ 0.159 & 0.428 $\pm$ 0.300 \\
%         & CNN   & 0.533 $\pm$ 0.123 & 0.520 $\pm$ 0.106 & 0.681 $\pm$ 0.206 & 0.358 $\pm$ 0.278 \\
%         & M2E & 0.638 $\pm$ 0.090 & 0.615 $\pm$ 0.237 & 0.663 $\pm$ 0.129 & 0.542 $\pm$ 0.318 \\
%         & MIC & 0.713 $\pm$ 0.129 & 0.704 $\pm$ 0.237 & 0.772 $\pm$ 0.146 & 0.650 $\pm$ 0.309 \\
%         & ITD-GCN & \textbf{0.833 $\pm$ 0.105} & \textbf{0.829 $\pm$ 0.121} & \textbf{0.856 $\pm$ 0.146} & \textbf{0.802 $\pm$ 0.191} \\
%    \specialrule{.1em}{.05em}{.05em}
%    \end{tabular}%
%  \label{Table_results_comparison}%
%\end{table*}%

% Table generated by Excel2LaTeX from sheet 'SimpleComparison'
% \begin{table*}[htbp]
% \tiny
%   \centering
%   \caption{Comparison with the state-of-the-art methods in terms of classification accuracy and AUC values (mean $\pm$ sd). The best and second best results are marked
% in red and blue, respectively.}
%     \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
%     \toprule
%     \multirow{3}[6]{*}{Datasets} & \multirow{3}[6]{*}{Metrics} & \multicolumn{10}{c|}{Methods} \\
% \cmidrule{3-12}          &       & \multicolumn{2}{c|}{PCA} & \multicolumn{2}{c|}{MPCA} & \multicolumn{2}{c|}{M2E} & \multicolumn{2}{c|}{MIC} & \multirow{2}[4]{*}{CNN} & \multirow{2}[4]{*}{IT-GCN} \\
% \cmidrule{3-10}          &       & KNN   & FCN   & KNN   & FCN   & KNN   & FCN   & KNN   & FCN   &       &  \\
%     \midrule
%     \multirow{2}[4]{*}{HIV} & accuracy & 0.686 $\pm$ 0.144 & 0.543 $\pm$ 0.194 & 0.643 $\pm$ 0.135 & 0.544 $\pm$ 0.139 & 0.586 $\pm$ 0.249 & 0.506 $\pm$ 0.137 & 0.571 $\pm$ 0.093 & 0.556 $\pm$ 0.153 & 0.546 $\pm$ 0.158 & 0.686 $\pm$ 0.131 \\
% \cmidrule{2-12}          & auc   & 0.672 $\pm$ 0.175 & 0.498 $\pm$ 0.167 & 0.622 $\pm$ 0.146 & 0.518 $\pm$ 0.047 & 0.553 $\pm$ 0.326 & 0.475 $\pm$ 0.057 & 0.577 $\pm$ 0.141 & 0.497 $\pm$ 0.224 & 0.541 $\pm$ 0.088 & 0.679 $\pm$ 0.099 \\
%     \midrule
%     \multirow{2}[4]{*}{BP} & accuracy & 0.544 $\pm$ 0.161 & 0.533 $\pm$ 0.187 & 0.522 $\pm$ 0.149 & 0.567 $\pm$ 0.063 & 0.644 $\pm$ 0.142 & 0.533 $\pm$ 0.123 & 0.522 $\pm$ 0.125 & 0.489 $\pm$ 0.127 & 0.533 $\pm$ 0.123 & 0.833 $\pm$ 0.105 \\
% \cmidrule{2-12}          & auc   & 0.543 $\pm$ 0.141 & 0.523 $\pm$ 0.133 & 0.528 $\pm$ 0.148 & 0.488 $\pm$ 0.037 & 0.639 $\pm$ 0.255 & 0.518 $\pm$ 0.069 & 0.532 $\pm$ 0.171 & 0.511 $\pm$ 0.028 & 0.521 $\pm$ 0.106 & 0.829 $\pm$ 0.121 \\
%     \bottomrule
%     \end{tabular}%
%   \label{Table_results_comparison}%
% \end{table*}%

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htbp]
\centering
\caption{Comparison with the state-of-the-art methods in terms of classification accuracy and AUC values (mean $\pm$ std). The best and second best results are marked
in red and blue, respectively.}
\resizebox{6.90in}{!}{%
\begin{tabular}{ccccclccccc}
\cline{1-5} \cline{7-11}
Dataset              & Group                 & Methods & Accuracy      & AUC           &  & Dataset             & Group                 & Methods & Accuracy      & AUC           \\ \cline{1-5} \cline{7-11}
\multirow{14}{*}{HIV} & \multirow{2}{*}{PCA}  & KNN    & 0.686 $\pm$ 0.164 & 0.672 $\pm$ 0.175 &  & \multirow{14}{*}{BP} & \multirow{2}{*}{PCA}  & KNN    & 0.544 $\pm$ 0.161 & 0.543 $\pm$ 0.141 \\
                     &                       & FCN    & 0.543 $\pm$ 0.194 & 0.498 $\pm$ 0.167 &  &                     &                       & FCN    & 0.533 $\pm$ 0.187 & 0.523 $\pm$ 0.133 \\ \cline{2-5} \cline{8-11} 
                     & \multirow{2}{*}{MPCA} & KNN    & 0.643 $\pm$ 0.135 & 0.622 $\pm$ 0.146 &  &                     & \multirow{2}{*}{MPCA} & KNN    & 0.522 $\pm$ 0.149 & 0.528 $\pm$ 0.148 \\
                     &                       & FCN    & 0.544 $\pm$ 0.139 & 0.518 $\pm$ 0.047 &  &                     &                       & FCN    & 0.567 $\pm$ 0.063 & 0.488 $\pm$ 0.037 \\ \cline{2-5} \cline{8-11} 
                     & \multirow{2}{*}{M2E}  & KNN    & 0.586 $\pm$ 0.249 & 0.553 $\pm$ 0.326 &  &                     & \multirow{2}{*}{M2E}  & KNN    & 0.644 $\pm$ 0.142 & 0.639 $\pm$ 0.255 \\
                     &                       & FCN    & 0.506 $\pm$ 0.137 & 0.475 $\pm$ 0.057 &  &                     &                       & FCN    & 0.533 $\pm$ 0.123 & 0.518 $\pm$ 0.069 \\ \cline{2-5} \cline{8-11} 
                     & \multirow{2}{*}{MIC}  & KNN    & 0.571 $\pm$ 0.093 & 0.577 $\pm$ 0.141 &  &                     & \multirow{2}{*}{MIC}  & KNN    & 0.522 $\pm$ 0.125 & 0.532 $\pm$ 0.171 \\
                     &                       & FCN    & 0.556 $\pm$ 0.153 & 0.497 $\pm$ 0.224 &  &                     &                       & FCN    & 0.489 $\pm$ 0.127 & 0.511 $\pm$ 0.028 \\ \cline{2-5} \cline{8-11} 
                     & \multirow{1}{*}{3D-CNN} & 3D-CNN    & 0.546 $\pm$ 0.158 & 0.541 $\pm$ 0.088 &  &                     & \multirow{1}{*}{3D-CNN} & 3D-CNN    & 0.533 $\pm$ 0.123 & 0.521 $\pm$ 0.106 \\ \cline{2-5} \cline{8-11} 
                     & \multirow{5}{*}{MVGCN} & RandomNode    & 0.629 $\pm$ 0.168 & 0.623 $\pm$ 0.130 &  &                     & \multirow{5}{*}{MVGCN} & RandomNode    & 0.778 $\pm$ 0.203 & 0.766 $\pm$ 0.216 \\
                     &                       & NodeAverage    & 0.671 $\pm$ 0.134 & 0.668 $\pm$ 0.161 &  &                     &                       & NodeAverage    & 0.822 $\pm$ 0.168 & 0.818 $\pm$ 0.101 \\
                    %  &                       & Node2Vec    & 0.671 $\pm$ 0.166 & 0.658 $\pm$ 0.152 &  &                     &                       & Node2Vec    & 0.833 $\pm$ 0.108 & 0.821 $\pm$ 0.114 \\ 
                     &                       & IT-GCN(CP)  & \textcolor{blue}{\textbf{0.686 $\pm$ 0.162}} & \textcolor{blue}{\textbf{0.675 $\pm$ 0.142}} &  &                     &                       & IT-GCN(CP)    & \textcolor{red}{\textbf{0.833  $\pm$ 0.094}} & \textcolor{red}{\textbf{0.829 $\pm$ 0.104}} \\ 
                     &                       & IT-GCN(Tucker) & \textcolor{red}{\textbf{0.686 $\pm$ 0.131}} & \textcolor{red}{\textbf{0.679 $\pm$ 0.099}} &  &                     &                       & IT-GCN(Tucker) & \textcolor{blue}{\textbf{0.833 $\pm$ 0.105}} & \textcolor{blue}{\textbf{0.829 $\pm$ 0.121}} \\ \cline{1-5} \cline{7-11} 
\end{tabular}
}
\label{Table_results_comparison}%
\end{table*}



% \begin{table}[htbp]
%   \centering
%   \caption{Ablation study on the influence of obtaining node embedding matrix with different methods.}
%   \resizebox{3.350in}{!}{%
%     \begin{tabular}{ccccc}
%     \toprule
%     Dataset & Method & Accuracy & AUC   & Time (s) \\
%     \midrule
%     \multirow{4}[8]{*}{HIV} & RandomNode-GCN & 0.629 $\pm$ 0.168 & 0.623 $\pm$ 0.130 & 0.06 \\
% \cmidrule{2-5}          & Node2Vec-GCN & 0.671 $\pm$ 0.166 & 0.658 $\pm$ 0.152 & $>$ 3600 \\
% \cmidrule{2-5}          & IT-GCN (CP) & \textbf{0.686 $\pm$ 0.162} & 0.675 $\pm$ 0.142 & 21.8 \\
% \cmidrule{2-5}          & IT-GCN & \textbf{0.686 $\pm$ 0.131} & \textbf{0.679 $\pm$ 0.099} & \textbf{0.18} \\
%     \midrule
%     \multirow{4}[8]{*}{BP} & RandomNode-GCN & 0.778 $\pm$ 0.203 & 0.766 $\pm$ 0.216 & 0.05 \\
% \cmidrule{2-5}          & Node2Vec-GCN & 0.833 $\pm$ 0.108 & 0.821 $\pm$ 0.114 & $>$ 3600 \\
% \cmidrule{2-5}          & IT-GCN (CP) & 0.833  $\pm$ 0.094 & 0.829 $\pm$ 0.104 & 15.4 \\
% \cmidrule{2-5}          & IT-GCN & \textbf{0.833 $\pm$ 0.105} & \textbf{0.829 $\pm$ 0.121} & \textbf{0.26} \\
%     \bottomrule
%     \end{tabular}%
%     }
%   \label{Table_ablation_node_embedding_matrix}%
% \end{table}%
